Admissible Hierarchical Clustering Methods and Algorithms for Asymmetric Networks

This paper characterizes hierarchical clustering methods that abide by two previously introduced axioms -- thus, denominated admissible methods -- and proposes tractable algorithms for their implementation. We leverage the fact that, for asymmetric networks, every admissible method must be contained between reciprocal and nonreciprocal clustering, and describe three families of intermediate methods. Grafting methods exchange branches between dendrograms generated by different admissible methods. The convex combination family combines admissible methods through a convex operation in the space of dendrograms, and thirdly, the semi-reciprocal family clusters nodes that are related by strong cyclic influences in the network. Algorithms for the computation of hierarchical clusters generated by reciprocal and nonreciprocal clustering as well as the grafting, convex combination, and semi-reciprocal families are derived using matrix operations in a dioid algebra. Finally, the introduced clustering methods and algorithms are exemplified through their application to a network describing the interrelation between sectors of the United States (U.S.) economy.

==> table_industrial_sectors.tex <==
%!TEX root = Asymmetric_Clustering_Journal_V_current.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% T A B L E         S E C T O R S %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand\arraystretch{1.2} 
\begin{table*}
\small
\centering
\caption{Code and description of industrial sectors}
\vspace{-0.1in}
\begin{tabular}{ l  l p{1cm}  l  l }
  \hline    
Code & Industrial Sector                                    &&%\\  \hline                     
Code & Industrial Sector                                    \\  \hline                    
AC & Accommodation                                          &&%\\ 
AG & Amusements, gambling, and recreation industries        \\ 
AH & Ambulatory health care services                        &&%\\ 
AP & Apparel and leather and allied products                \\ 
AT & Air transportation                                     &&%\\ 
AS & Administrative and support services                    \\ 
BT & Broadcasting and telecommunications                    &&%\\ 
CE & Computer and electronic products                       \\ 
CH & Chemical products                                      &&%\\ 
CO & Construction                                           \\ 
CS & Computer systems design and related services           &&%\\ 
ED & Educational services                                   \\ 
EL & Electrical equipment, appliances, and components       &&%\\ 
FA & Farms                                                  \\ 
FB & Food and beverage and tobacco products                 &&%\\ 
FO & Forestry, fishing, and related activities              \\ 
FM & Fabricated metal products                              &&%\\ 
FR & Federal Reserve banks and credit intermediation        \\ 
FU & Furniture and related products                         &&%\\ 
FP & Food services and drinking places                      \\ 
FT & Funds, trusts, and other financial vehicles            &&%\\ 
IC & Insurance carriers and related activities              \\ 
ID & Information and data processing services               &&%\\ 
LS & Legal services                                         \\ 
MI & Mining, except oil and gas                             &&%\\ 
MA & Machinery                                              \\ 
MV & Motor vehicles, bodies and trailers, and parts         &&%\\ 
MC & Management of companies and enterprises                \\ 
MM & Miscellaneous manufacturing                            &&%\\ 
MP & Misc. professional, scientific, and technical services \\ 
NM & Nonmetallic mineral products                           &&%\\ 
OG & Oil and gas extraction                                 \\ 
OS & Other services, except government                      &&%\\ 
OT & Other transportation and support activities            \\ 
PA & Paper products                                         &&%\\ 
PC & Petroleum and coal products                            \\ 
PE & Performing arts, spectator sports and museums          &&%\\ 
PL &Plastics and rubber products                            \\ 
PM & Primary metals                                         &&%\\ 
PR & Printing and related support activities                \\ 
PS & Motion picture and sound recording industries          &&%\\ 
PT & Pipeline transportation                                \\ 
PU & Publishing industries (includes software)              &&%\\ 
RA & Real estate                                            \\ 
RE & Retail trade                                           &&%\\ 
RL & Rental and leasing serv. and lessors of intang. assets \\ 
RT & Rail transportation                                    &&%\\ 
SA & Social assistance                                      \\ 
SC & Securities, commodity contracts, and investments       &&%\\ 
SM & Support activities for mining                          \\ 
TE & Textile mills and textile product mills                &&%\\ 
TG & Transit and ground passenger transportation            \\ 
TM & Other transportation equipment                         &&%\\ 
TT & Truck transportation                                   \\ 
UT & Utilities                                              &&%\\ 
WH & Wholesale trade                                        \\ 
WM & Waste management and remediation services              &&%\\ 
WO & Wood products                                          \\ 
WT & Water transportation                                   &&%\\ 
WS & Warehousing and storage                                \\ \hline





\end{tabular}
\label{table_industrial_sectors}
\vspace{-0.1in}
\end{table*}




